Developer Experiences with Cursor AI-native IDE

AI-powered integrated development environments (IDEs) are increasingly positioned as practical tools for software development, integrating AI assistance into everyday activities such as editing, refactoring, and debugging. However, how developers evaluate AI IDEs as working environments, what frictions shape their adoption, and which aspects of the experience matter most in everyday use remain underexplored. Prior evidence on adoption and use is mainly controlled tasks, small interview samples, and short observation windows, which offer limited visibility into longitudinal, community-driven experience and the workflow drift that emerges in everyday practice. To bridge this gap, we conduct a large-scale longitudinal study of Cursor, a prominent AI-native IDE, through its official public forum, where users report bugs, request features, and discuss everyday use. Our analysis covers 14,714 forum posts collected over more than two years. We find that discussion is dominated by workflow-critical mechanisms (71%) such as context indexing, model routing, and agent workflows, which are also the main sources of both perceived value and frustration. Negative experiences center on usability, pricing, and dependability, including installation and setup, usage limits and consumption, crashes, and latency. Over time, the focus of friction shifts from early access and setup barriers toward pricing, robustness, and sustained workflow reliability.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf


all:  ${PDF}
	cd samples && ${MAKE} $@

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<

%-tagged.cls:   %.ins %.dtx
	pdflatex $<


tagged:
	${MAKE} acmart.cls && cd samples && ${MAKE} acmsmall-tagged.pdf && ${MAKE} sigconf-tagged.pdf




.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls $(PACKAGE)-tagged.cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi
	cd samples && ${MAKE} $@


clean: docclean
	$(RM)  $(PACKAGE).cls $(PACKAGE)-tagged.cls 
	cd samples && ${MAKE} $@

distclean: clean
	$(RM)  *.pdf 
	cd samples && ${MAKE} $@

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' --exclude LICENSE $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

# distros
distros: all docclean
	zip -r acm-distro.zip  \
	acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.* LICENSE \
	--exclude samples/sample-acmengage*
	zip -r acmengage-distro.zip samples/sample-acmengage* LICENSE \
	samples/*.bib \
	acmart.pdf acmguide.pdf  *.cls ACM-Reference-Format.*

acmcp.zip: all acmart.cls
	zip $@ $+



==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

Version 2.19   2026-06-27
               Re-added keywords to samples
	       Tagging: defaults for tables
	       Bug fixes

Version 2.18   2026-05-31
               Bug fixes
	       Deleted IMS designation from journals
	       Deprecated keywords
	       Bibliography change: moved note before URL
	       Merged tagging code into the main branch.
	       New code for captions in the tagging version.
	       

Version 2.17   2026-03-28
	       Bugs fixed

Version 2.16   2025-08-27
	       Emergency release: fixes a typo in the code.


Version 2.15   2025-08-21
	       Bug fixes.  Documentation updates
	       New journals: AILET, TAIS, TAISAP, ACMJDS

Version 2.14   2025-05-30
	       Bib style update.  Documentation update.  DLT is now using
	       acmlarge format.
	       Generate error if a user tries to redefine sectioning commands

Version 2.13   
               Documentation update
	       Added mathcal in unicode mode
	       Bug fixes

Version 2.12   2024-12-31
	       Bug fixes
	       Switched to unicode-math and libertinus for Unicode engines

Version 2.11   2024-12-21
	       Conference date is no longer printed in bibstrip.
	       ISBN now uses 4-digit year
	       DOI in bibliography is now output as doi:XX.XXXX/XXXXX.XXXX
	       Changed URL in Creative Commons licenses (deleted
	       trailing /legalcode)

Version 2.10.  2024-10-19
	       Bug fixes.  Documentation update.

Version 2.09   2024-08-25
	       Experimental tagging code is now in the main branch.
	       Creative Commons license is now allowed for all materials. 

Version 2.08   2024-06-01
	       Section titles are in lowercase now.
	       Documentation updates.

Version 2.07   2024-04-17
	       Corrected typo in TELO eISSN.

Version 2.06   2024-04-13
	       Added eISSN for a number of journals.
               ACM no longer collects or prints authors'
	       postal addresses

Version 2.05   2024-04-04
	       Changed title for TELO.

Version 2.04   2024-03-31
	       Compatibility with the new latex-dev format
               eSSN is always printed, even if pSSN is present
	       Wording change in copyright statement

Version 2.03   2024-02-04
	       Cleaned generation of samples.
	       New options for printing conference proceedings
	       in ACM journals

Version 2.02   2024-01-21
	       Documentation update.
	       Changes in TOG templates
	       Corrected typo in ACM/IMS journals

Version 2.01   2023-12-29
	       \acmPrice now produces a warning.

Version 2.00   2023-11-08
	       ACM switches to electronic only version.
	       We do not print article tabs anymore.
	       New copyright wording.
	       Deleted \acmPrice.

Version 1.93   Added PACMSE

Version 1.92   Documentation update
	       Emergency change: changed order of hyperref and hyperxmp
	       due to changes in the undelying packages

Version 1.91   Minor changes in ACMCP format

Version 1.90a  Changes in the sample keywords and concepts

Version 1.90   Journal ISSN updated

Version 1.89a  Added version info to .bst

Version 1.89   Bug fixes
	       Redesign of ACMCP
	       New positioning of badges
	       New journals: PACMMOD, TOPML

Version 1.88   New ISSNs
	       Documentation updates
	       New journal:  PACMNET

Version 1.87   CC license is allowed for non-acm documents and ACM Engage
	       documents only
	       New format acmcp for the cover page
	       New journals: JATS, ACMJCSS, TORS
	       Bug fixes

Version 1.86.  Empty country in affiliation now produces an error
               Bug fixes
	       New samples for acmengage

Version 1.85.  Bug fixes
	       Added support for Creative Commons licenses (requires
	       doclicense images)
	       New journals
	       New format acmengage for ACM Engage CSEdu course materials 

Version 1.84   Support for BibLaTeX rewritten (thanks to
	       Roberto Di Cosmo and Kartik Singhal)
	       Corrected German translation (thanks to Dirk Beyer)
	       New journals

Version 1.83   Support for multilanguage papers
	       ISSN changes for some journals

Version 1.82   Bug fixes.
	       New command \anon for anonymization of short strings.
	       Documentation update.

Version 1.81   Bug fixes
	       New bib field distinctURL to print URL even if doi is present.
	       Reworded samples

Version 1.80   New journals: DLT, FAC

Version 1.79   Fixed pages with index
	       (https://github.com/borisveytsman/acmart/issues/440)
	       Updated information for TAP, TCPS, TEAC

Version 1.78   Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.

Version 1.77   Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.76   Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.75   Omitted \country now produces error.
	       Added \AtBeginMaketitle

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations.  The absence of them produces a warning

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.63a   Moved TQUANT to TQC

Version 1.63	New journals: TQUANT, FACMP

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.52    Another rewording of licenses

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.49    New jorunal:  DTRAP

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.47    New journal: THRI

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.43    Bug fixes

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.41    Rearranged bib files
                Added new badges

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.39    Added \authornotemark commmand

Version 1.38    Increase default font size for SIGPLAN

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

Version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

Version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

Version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

Version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

Version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

Version 1.28    Bug fixes: natbib=false now behaves correctly.

Version 1.27    Bug fixes

Version 1.26    Bug fixes

Version 1.25    Updated PACMPL journal option.

Version 1.24    Added IMWUT journal option.

Version 1.23    Added PACM PL journal option.

Version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

Version 1.21    Bibliography changes: added arXiv, some cleanup

Version 1.20    Bug fixes, documentation updates

Version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

Version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.


Version 1.17    Formatting changes for margins and lists.  Bug fixes.

Version 1.16    Formatting changes for headers and footers.

Version 1.15    New structured affiliation command.
                New commands for acknowledgements.

Version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

Version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

Version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

Version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

Version 1.10    Bug fixes

Version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

Version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes


==> figure/agent.tex <==
\begin{figure}[t]
  \centering
  \includegraphics[width=0.48\textwidth]{figure/trust-agent.png}
  \caption{A common workflow of SE agents}
  \label{fig:agent}
\end{figure}

==> figure/comparison_over_time.tex <==
\begin{figure}[t]
  \centering  \includegraphics[width=0.50\textwidth]{figure/rq4_comparison_over_time.png}
  \caption{Comparison posts over time. Stacked bars show the composition of comparison subcategories each quarter (share of comparison posts), while the overlaid line shows the total number of comparison posts per quarter.}  \label{fig:comparsion_overtime}
\end{figure}


==> figure/cursor_webpage.tex <==
\begin{figure}[t]
  \centering  \includegraphics[width=0.50\textwidth]{figure/Cursor_webpage.png}
  \caption{The screenshot of the appearance of Cursor's webpage. }
  \label{fig:webpage}
\end{figure}


==> figure/neg_over_time.tex <==
\begin{figure}[t]
  \centering
  \includegraphics[width=0.50\textwidth]{figure/negative_over_time.png}
  \caption{\textbf{Negative posts: popularity, agreement and engagement over time.}
Quarterly averages computed over negative posts. Popularity is mean views per post (left y-axis); agreement (mean likes) and engagement (mean replies/comments) are plotted on a separate y-axis (right) due to scale differences. Gray bars indicate the number of negative posts per quarter.}
  \label{fig:neg_over_time}
\end{figure}


==> figure/popularity_heatmap.tex <==
\begin{figure}[t]
  \centering
  \includegraphics[width=0.50\textwidth]{figure/rq3_topic_trends_category_popularity_heatmap.png}
  \caption{Category-level attention per negative post over time (popularity heatmap)}
  \label{fig:popularity_heatmap}
\end{figure}

% what complaints attract the most attention per post

==> figure/popularity_trend.tex <==
\begin{figure}[t]
  \centering
  \includegraphics[width=0.48\textwidth]{figure/stack_area.png}
  \caption{Category-level composition of negative posts by quarter (counts; normalized to 100\%)}
  \label{fig:topic_trends}
\end{figure}

% what people complain about most often

==> figure/pos_share_like.tex <==
\begin{figure}[t]
  \centering
  \includegraphics[width=0.50\textwidth]{figure/share-like.png}
  \caption{\textbf{Positive posts: share of likes by category over time.} Stacked areas show, for each quarter, the fraction of total likes on positive posts attributable to each category (shares sum to 1.0 per quarter).}
  \label{fig:pos_share_like}
\end{figure}


==> figure/pos_share_replies.tex <==
\begin{figure}[t]
  \centering
  \includegraphics[width=0.50\textwidth]{figure/share-reply.png}
  \caption{\textbf{Positive posts: share of replies by category over time.}
Stacked areas show, for each quarter, the fraction of total replies/comments on positive posts attributable to each category (shares sum to 1.0 per quarter).}
  \label{fig:pos_share_reply}
\end{figure}


==> figure/pos_share_view.tex <==
\begin{figure}[t]
  \centering
  \includegraphics[width=0.50\textwidth]{figure/share-views.png}
  \caption{\textbf{Positive posts: share of views by category over time.}
Stacked areas show, for each quarter, the fraction of total views on positive posts attributable to each category (shares sum to 1.0 per quarter).}
  \label{fig:pos_share_view}
\end{figure}


==> figure/positive_over_time.tex <==
\begin{figure}[t]
  \centering  \includegraphics[width=0.50\textwidth]{figure/positive_over_time.png}
  \caption{\textbf{Positive posts: popularity, agreement and engagement over time.}
Quarterly averages computed over positive posts. Popularity is mean views per post (left y-axis); agreement (mean likes) and engagement (mean replies/comments) are plotted on a separate y-axis (right) due to scale differences. Gray bars indicate the number of positive posts per quarter.}
  \label{fig:pos_over_time}
\end{figure}


==> macros.tex <==
\usepackage{soul}
%\usepackage{times}
%\usepackage[T1]{fontenc}
%\usepackage{lmodern}
\usepackage{hyperref}
\usepackage{multirow}
\usepackage{listings}
\usepackage{fancybox}
\usepackage{enumitem}
\usepackage{graphicx}
%\usepackage{paralist}
%\usepackage{framed}
%\usepackage{multicols}
\usepackage{color}
%\usepackage{xcolor}
\usepackage{array}
\usepackage{amsmath}
\usepackage{xspace}
\usepackage{url}
\usepackage{tikz}
% \usepackage{caption}
\usepackage{pgfplots}
\usepackage{balance}
\usepackage{subcaption}
\captionsetup[figure]{font=footnotesize}
\captionsetup[table]{font=footnotesize}
\pgfplotsset{compat=1.16}
\usepackage{pgf-pie}
%\usepackage[table]{xcolor}
\RequirePackage{colortbl}
\usepackage{booktabs}
\usepackage{ragged2e} % for \RaggedRight
\newcolumntype{Y}{>{\RaggedRight\arraybackslash}X}
\usetikzlibrary{pgfplots.statistics,calc}
\usepackage{algorithm}
\usepackage{algorithmic}
\usepackage{adjustbox}
\usepackage{makecell}
\usepackage{tabularx}
\usetikzlibrary{calc}
\usepackage{tikz}
\usepackage{csquotes}
\newcommand*\circled[1]{\tikz[baseline=(char.base)]{
            \node[shape=circle,draw,inner sep=2pt] (char) {#1};}}

\clubpenalty=100000000 %10000
\widowpenalty=10000000 %10000
\brokenpenalty=10000000 %10000

\usepackage{tcolorbox}
% \makeatletter
% \newcommand{\mybox}[1]{%
% 	\setbox0=\hbox{#1}%
% 	\setlength{\@tempdima}{\dimexpr\wd0+13pt}%
% 	\begin{tcolorbox}[boxrule=0.5pt, colback=white, arc=4pt,
% 		left=6pt,right=6pt,top=6pt,bottom=6pt,boxsep=0pt]
% 		#1
% 	\end{tcolorbox}
% }
\usepackage{pgfplotstable}
%
% observation box
% Preamble
% \usepackage[most]{tcolorbox}

\newcounter{observation}
\newtcolorbox{observationbox}[1][]{
  colback=white,
  colframe=black!60,
  boxrule=0.6pt,
  arc=2pt,
  left=6pt,right=6pt,top=4pt,bottom=4pt,
  fonttitle=\bfseries,
  title={Observation~\stepcounter{observation}\theobservation},
  #1
}

\newcommand{\tikzcircle}[2][red,fill=red]{\tikz[baseline=-0.5ex]\draw[#1,radius=#2] (0,0) circle ;}%

\definecolor{songcolor}{RGB}{191,191,191}
\newcommand{\todoc}[2]{{\textcolor{#1}{\textbf{#2}}}}
% todo commands:
\newcommand{\todored}[1]{\todoc{red}{\textbf{[[#1]]}}}
\newcommand{\todogreen}[1]{\todoc{green}{\textbf{[[#1]]}}}
\newcommand{\todoblue}[1]{\todoc{blue}{\textbf{[[#1]]}}}
\newcommand{\todogray}[1]{\todoc{Gray}{\textbf{[[#1]]}}}
\newcommand{\todoorange}[1]{\todoc{orange}{\textbf{[[#1]]}}}
\newcommand{\todobrown}[1]{\todoc{brown}{\textbf{[[#1]]}}}
\newcommand{\todopurple}[1]{\todoc{purple}{\textbf{[[#1]]}}}
\newcommand{\todoamber}[1]{\todoc{teal}{\textbf{[[#1]]}}}
%
%\newcommand{\tikzcircle}[2][red,fill=red]{\tikz[baseline=-0.5ex]\draw[#1,radius=#2] (0,0) circle ;}%


\newcommand{\add}[1]{\todoblue{#1}}
\newcommand{\todo}[1]{\todogreen{TODO: #1}}
\newcommand{\song}[1]{\todored{Song: #1}}
\newcommand{\gias}[1]{\todopurple{Gias: #1}}
\newcommand{\haoran}[1]{\todoorange{Haoran: #1}}
% \newcommand{\sentbar}[3]{%
% \begin{tikzpicture}[scale=0.8,baseline]
%   \fill[green!70] (0,0) rectangle (#1,0.3);
%   \fill[gray!60] (#1,0) rectangle (#1+#2,0.3);
%   \fill[red!70]  (#1+#2,0) rectangle (#1+#2+#3,0.3);
%   \draw[black!60] (0,0) rectangle (#1+#2+#3,0.3);
% \end{tikzpicture}%
% }

\newcolumntype{Y}{>{\raggedright\arraybackslash\hsize=0.85\hsize}X} % Category-Subcategory
\newcolumntype{Z}{>{\raggedright\arraybackslash\hsize=1.15\hsize}X} % Description

% Colors
\definecolor{sentpos}{RGB}{92,170,97}    % positive
\definecolor{sentneu}{RGB}{220,220,220}  % neutral
\definecolor{sentneg}{RGB}{227,90,83}    % negative
% \newlength{\SentBarW}\setlength{\SentBarW}{3.55cm}
% \newlength{\SentBarH}\setlength{\SentBarH}{0.22cm}
% \newlength{\SentBarX}\setlength{\SentBarX}{0.82cm}  % bar starts after left number
% \newlength{\SentGap}\setlength{\SentGap}{0.06cm}    % gap before right number


% % #1 pos, #2 neu, #3 neg
% \newcommand{\sentbar}[3]{%
% \begingroup
%   \pgfmathsetmacro{\PosRaw}{#1}
%   \pgfmathsetmacro{\NeuRaw}{#2}
%   \pgfmathsetmacro{\NegRaw}{#3}
%   \pgfmathsetmacro{\Sum}{\PosRaw+\NeuRaw+\NegRaw}
%   \pgfmathsetmacro{\Pos}{ifthenelse(\Sum>0,\PosRaw/\Sum,0)}
%   \pgfmathsetmacro{\Neu}{ifthenelse(\Sum>0,\NeuRaw/\Sum,0)}
%   \pgfmathsetmacro{\Neg}{ifthenelse(\Sum>0,\NegRaw/\Sum,0)}

%   % lengths
%   \pgfmathsetlengthmacro{\wPos}{\Pos*\SentBarW}
%   \pgfmathsetlengthmacro{\wNeu}{\Neu*\SentBarW}
%   \pgfmathsetlengthmacro{\wNeg}{\Neg*\SentBarW}
%   \pgfmathsetlengthmacro{\xNeu}{\Pos*\SentBarW}
%   \pgfmathsetlengthmacro{\xNeg}{(\Pos+\Neu)*\SentBarW}

%   % left/right percentages (no neutral number)
%   \pgfmathsetmacro{\pPct}{100*\Pos}
%   \pgfmathsetmacro{\dPct}{100*\Neg}

% \begin{tikzpicture}[baseline=(base)]
%   \coordinate (base) at (0,0);

%   % Bar start (MUST come before any use of (b))
%   \coordinate (b) at (\SentBarX,0);

%   % Force identical total width for every row (put early)
%   \path[use as bounding box] (0,-0.6\SentBarH) rectangle (\SentPicW,0.6\SentBarH);

%   % Positive (left) — close to bar
%   \node[anchor=east,inner sep=0pt,outer sep=0pt,font=\scriptsize,text=sentpos]
%     at ($(b)+(-\SentGap,0)$) {\pgfmathprintnumber[fixed,precision=1]{\pPct}\%};

%   % Stacked bar
%   \path[fill=sentpos] ($(b)+(0,-0.5\SentBarH)$) rectangle ++(\wPos,\SentBarH);
%   \path[fill=sentneu] ($(b)+(\xNeu,-0.5\SentBarH)$) rectangle ++(\wNeu,\SentBarH);
%   \path[fill=sentneg] ($(b)+(\xNeg,-0.5\SentBarH)$) rectangle ++(\wNeg,\SentBarH);

%   % Outline
%   \draw[black!35,line width=0.2pt] ($(b)+(0,-0.5\SentBarH)$) rectangle ++(\SentBarW,\SentBarH);

%   % Negative (right)
%   \node[anchor=west,inner sep=0pt,outer sep=0pt,font=\scriptsize,text=sentneg]
%     at ($(b)+(\SentBarW+\SentGap,0)$) {\pgfmathprintnumber[fixed,precision=1]{\dPct}\%};
% \end{tikzpicture}%


% % Legend for the bottom row (use inside the table)
% \newcommand{\sentlegend}{%
% \raisebox{0.2ex}{\tikz{\fill[sentpos] (0,0) rectangle (0.32,0.18);}}\;Positive\quad
% \raisebox{0.2ex}{\tikz{\fill[sentneu] (0,0) rectangle (0.32,0.18);}}\;Neutral\quad
% \raisebox{0.2ex}{\tikz{\fill[sentneg] (0,0) rectangle (0.32,0.18);}}\;Negative%
% }


\newlength{\SentBarW}\setlength{\SentBarW}{1.8cm}
\newlength{\SentBarH}\setlength{\SentBarH}{0.2cm}
\newlength{\SentBarX}\setlength{\SentBarX}{0.6cm}  % bar starts after left number
\newlength{\SentGap}\setlength{\SentGap}{0.06cm}    % gap before right number

% Fixed picture width (for identical alignment across rows)
\newlength{\SentPicW}
\setlength{\SentPicW}{\dimexpr\SentBarX+\SentBarW+1.00cm\relax} % extra room for right label

% #1 pos, #2 neu, #3 neg  (inputs can be raw or already-normalized)
\newcommand{\sentbar}[3]{%
\begingroup
  \pgfmathsetmacro{\PosRaw}{#1}
  \pgfmathsetmacro{\NeuRaw}{#2}
  \pgfmathsetmacro{\NegRaw}{#3}
  \pgfmathsetmacro{\Sum}{\PosRaw+\NeuRaw+\NegRaw}
  \pgfmathsetmacro{\Pos}{ifthenelse(\Sum>0,\PosRaw/\Sum,0)}
  \pgfmathsetmacro{\Neu}{ifthenelse(\Sum>0,\NeuRaw/\Sum,0)}
  \pgfmathsetmacro{\Neg}{ifthenelse(\Sum>0,\NegRaw/\Sum,0)}

  % lengths
  \pgfmathsetlengthmacro{\wPos}{\Pos*\SentBarW}
  \pgfmathsetlengthmacro{\wNeu}{\Neu*\SentBarW}
  \pgfmathsetlengthmacro{\wNeg}{\Neg*\SentBarW}
  \pgfmathsetlengthmacro{\xNeu}{\Pos*\SentBarW}
  \pgfmathsetlengthmacro{\xNeg}{(\Pos+\Neu)*\SentBarW}

  % left/right percentages (show pos and neg; neutral has no number)
  \pgfmathsetmacro{\pPct}{100*\Pos}
  \pgfmathsetmacro{\dPct}{100*\Neg}

\begin{tikzpicture}[baseline=(base)]
  \coordinate (base) at (0,0);
  \coordinate (b) at (\SentBarX,0);

  % Force identical total width for every row
  \path[use as bounding box] (0,-0.6\SentBarH) rectangle (\SentPicW,0.6\SentBarH);

  % Positive (left)
  \node[anchor=east,inner sep=0pt,outer sep=0pt,font=\scriptsize,text=sentpos]
    at ($(b)+(-\SentGap,0)$) {\pgfmathprintnumber[fixed,precision=1]{\pPct}\%};

  % Stacked bar
  \path[fill=sentpos] ($(b)+(0,-0.3\SentBarH)$) rectangle ++(\wPos,\SentBarH);
  \path[fill=sentneu] ($(b)+(\xNeu,-0.3\SentBarH)$) rectangle ++(\wNeu,\SentBarH);
  \path[fill=sentneg] ($(b)+(\xNeg,-0.3\SentBarH)$) rectangle ++(\wNeg,\SentBarH);

  % Outline
  \draw[black!35,line width=0.2pt] ($(b)+(0,-0.3\SentBarH)$) rectangle ++(\SentBarW,\SentBarH);

  % Negative (right)
  \node[anchor=west,inner sep=0pt,outer sep=0pt,font=\scriptsize,text=sentneg]
    at ($(b)+(\SentBarW+\SentGap,0)$) {\pgfmathprintnumber[fixed,precision=1]{\dPct}\%};
\end{tikzpicture}%
\endgroup
}

% Legend (use in a bottom row / note cell)
\newcommand{\sentlegend}{%
\raisebox{0.2ex}{\tikz{\fill[sentpos] (0,0) rectangle (0.32,0.18);}}\;Positive\quad
\raisebox{0.2ex}{\tikz{\fill[sentneu] (0,0) rectangle (0.32,0.18);}}\;Neutral\quad
\raisebox{0.2ex}{\tikz{\fill[sentneg] (0,0) rectangle (0.32,0.18);}}\;Negative%
}


\newcommand{\cursor}{\textit{Cursor}}

\newcommand{\review}[1]{{\textit{#1}}~\\}
\newcommand{\respto}[1]{
\fcolorbox{black}{black!15}{
\label{response:#1}
\bf
  \scriptsize Review {#1}}~
}
\newcommand{\citerespexp}[1]{
\fcolorbox{black}{black!15}{
 \bf
  \scriptsize Review {#1}}~{\bf{on page \pageref{response:#1}}}
}

\newcommand{\citeresp}[1]{
\fcolorbox{black}{black!15}{
 \bf
  \scriptsize Review {#1}}
}


% --- for revision
\newcommand{\rev}[1]{\textcolor{purple}{\st{#1}}}
%\newcommand{\rev}[1]{}
%\newcommand{\add}[1]{\textcolor{blue}{{#1}}

%% space in some tables.  BUT have it here, such that you can always renew it
\newcommand{\ts}{$\;$}
\newcommand{\tS}{$\;$}
\newcommand{\tts}{\ \ \ \ \ }
\newcommand{\tss}{\ \ \ $\;$}
\newcommand{\ttts}{$\;$}
\newcommand{\decentHLine}{\noalign{\hrule height 1.04pt}}

==> sections/RQ4.tex <==
\subsection{RQ4. Comparison {\cursor} with Other Tools}
\subsubsection{Approach}
In this section, we examine the Comparison category in detail to understand what other tools developers use as reference points for evaluating {\cursor}, and what these comparisons reveal about adoption and expectations.

\subsubsection{Results}
Across the full corpus of 14714 posts, 416 posts (2.8\%) are labeled under Comparison in Table~\ref{category_list}, among these, 69.7\% is about comparing {\cursor} with VS code, 21.9\% are about comparing {\cursor} with AI coding assistants, 5.5\% comparing with traditional IDEs, and 2.9\% are about comparing with other AI-first IDEs. 
% Comparison discussions are also measurably more visible than typical forum threads. Comparison posts receive a mean of 1{,}230 views per thread, versus 747 views for non-comparison posts. However, they receive fewer likes on average (2.7 vs.\ 3.5), suggesting that comparison threads function less as endorsement and more as shared evaluation artifacts. Attention is also strongly concentrated: the top 10\% most-viewed comparison threads account for 67.1\% of all views accumulated by comparison posts, the top 5\% account for 52.3\%, and the top 1\% account for 25.6\%. These concentration levels indicate that a small number of high-salience threads become canonical references that many readers consult during adoption and toolchain decisions.
\input{tabs/comparison_dimension}
\input{figure/comparison_over_time}

Figure~\ref{fig:comparsion_overtime} traces comparison discourse using both its absolute volume (line) and its topic mix (100\% stacked bars). In the first year of the forum, cross-tool comparisons are present but remain modest and fluctuating, moving from 12 posts (2023Q3) to 25 (2023Q4), then hovering around 22 (2024Q1) and 15 (2024Q2). During this low-volume phase, the composition still shows a clear baseline anchor that most comparisons are framed against VS Code (72–75\% in 2023Q3–2023Q4 and 73.3\% in 2024Q2), reflecting {\cursor}’s proximity to VS Code workflows and the practical migration questions that follow. The main exception is 2024Q1, where the discussion becomes evenly split between VS Code (50.0\%) and AI coding assistants (50.0\%), suggesting a moment when users treated the decision less as “editor replacement” and more as “assistant vs. IDE-integrated AI” positioning. Comparison threads increase to 65 posts in 2024Q3, and the conversation remains elevated through 2025Q3 (66 in 2024Q4, 68 in 2025Q1, 58 in 2025Q2, 62 in 2025Q3). Notably, comparisons to VS Code continue to dominate most quarters in this high-volume regime (78.5\% in 2024Q3, 75.8\% in 2024Q4, 70.6\% in 2025Q1), indicating that as adoption broadens, users repeatedly return to VS Code parity and integration as the reference point. However, the stacked bars also show that the secondary comparison targets become more dynamic after the surge. There are two notable patterns. First, comparisons to traditional IDEs and editors remain a persistent but smaller stream, rising to 13.3\% (2024Q2) and 11.8\% (2025Q1). Second, the forum compares {\cursor} with other AI-first IDEs only in the later period: while nearly absent earlier (0.0\% through 2024Q4, 1.5\% in 2025Q1), this category spikes sharply in 2025Q2 (15.5\%), before receding again (3.2\% in 2025Q3, 0.0\% in 2025Q4). This brief but significant rise indicates an emerging peer set and a shift from “{\cursor} vs. legacy baseline” to “{\cursor} vs. competing AI-first IDE designs,” consistent with a market phase where users evaluate among similar paradigms rather than against traditional toolchains. The drop in 2025Q4 should not be interpreted as the comparison conversation “cooling off” in any substantive sense. Instead, it is better read as consolidation: by late 2025, cross-tool evaluation appears to have produced a small set of high-salience, reusable threads that newcomers consult rather than repeatedly recreate. More importantly, 2025Q4’s composition indicates which evaluation axes remain structurally unresolved. Even in a low-volume quarter, the conversation snaps back to the durable baseline, roughly 17 of 23 threads comparing with VS Code (73.9\%) and ~5 comparing with AI assistants (21.7\%), which suggests that the community’s long-run decision problem is still dominated by (i) migration and ecosystem parity relative to the de facto workflow substrate (VS Code) and (ii) value and assistance-quality tradeoffs relative to standalone assistants. The brief emergence of “other AI-first IDE” comparisons earlier then reads more like a competitive shock that temporarily broadens the reference set. Taken together, comparison discourse continues to foreground the same two adoption-critical questions: whether {\cursor} can behave as a drop-in, low-friction extension of an existing VS Code-centered toolchain, and whether its AI-native workflow delivers enough incremental benefit to justify switching costs versus assistant-only alternatives.

Figure~\ref{fig:comparison_subcategory_pies} further shows the specific aspects that users compare. When {\cursor} is compared with VS Code (13a), the discussion concentrates on interaction surface (23.1\%) and ecosystem fit (21.4\%) because {\cursor} is built on the VS Code codebase and inherits its interaction model and windowing structure, making the comparison primarily about whether {\cursor} preserves VS Code’s familiar operating experience while adding AI capabilities and where that inheritance breaks down in practice. However, only about one-tenth of threads favor {\cursor} on the these two most salient aspects (10.4\% for interaction surface and 11.3\% for ecosystem fit), whereas the large majority favor the incumbent (89.6\% and 88.7\%, respectively), representing that users wish to keep the features that available in the VS Code and can work along with {\cursor} well. In that framing, users are effectively asking whether {\cursor} can serve as a credible “primary IDE” without imposing friction: layout, navigation, and interaction conventions become salient because even small deviations compound across hours of use, and extension and integration talk reflects the practical switching cost of losing a mature toolchain. The comparison, therefore, emphasizes compatibility and workflow continuity rather than model quality alone; users are not evaluating {\cursor} as a novel AI feature, but as a replacement for a heavily customized environment. This also explains why terminal and remote-development aspects appear prominently in this target: once the baseline is an IDE, stability in the “full-stack” developer loop (editing, running, debugging, remote contexts) becomes the decisive criterion for adoption. The figure also shows users' attitude through comparison of whether they prefer {\cursor} or VS Code. 

When {\cursor} is compared with traditional IDEs/editors (i.e., JetBrains IDEs), the comparison is more framed around classic IDE competencies, such as editor features, debugging, and tooling, and the aspect distribution reflects that shift. Here, the attention clusters around ecosystem integration (26.1\%) and editor/coding experience (21.8\%), where denotes core IDE behaviors such as autocomplete, diffs, diagnostics, navigation, testing, and language support. Notably, the only area where {\cursor} is favored is the ecosystem layer (66.7\% prefer {\cursor} vs. 33.3\% prefer the opponent). By contrast, the preference for core IDE surfaces leans heavily toward the traditional baseline.  When users compare {\cursor} with AI-coding assistants and other AI-first IDEs, model-related aspects such as model availability, routing, and selection become the major aspects users mentioned (16.5\% and 33.3\% respectively). Users also report positive experiences with coding, pricing plans, API connectivity, and AI coding assistants (such as Copilot, Claude Code), and other AI-driven IDEs that {\cursor} can learn from and adopt. In the meantime, users also reflect {\cursor} with a better experience on the usage workflow and more productivity. 

\input{figure/comparison_breakdown}


\begin{observationbox}
Developers evaluate {\cursor} as a potential replacement for a heavily customized VS Code-centered toolchain. Expectations are therefore dominated by “drop-in” workflow continuity: interaction surface, extension/tooling parity, and avoiding migration pain.
\end{observationbox}

\begin{observationbox}
The comparison standards shift by reference point: against traditional IDEs, focus is on core IDE competencies and ecosystem integration;
% and {\cursor} is mainly credited at the ecosystem layer; 
against AI assistants and AI-first IDEs, focus pivots to model availability, routing/selection, alongside pricing plan, and API connectivity. 
% This indicates that adoption expectations extend beyond editor replacement toward AI-native workflow value, while switching costs span both IDE competencies, tooling depth and the model layer’s controllability and value tradeoffs.   
\end{observationbox}

==> sections/related.tex <==
\section{Related Works}
\label{sec:related}

==> tabs/comparison_dimension.tex <==
\begin{table}[t]
\caption{Comparison aspects in Comparison posts grouped by the original taxonomy category (share of comparison posts by original category, sentiment composition, and mean engagement).}
\label{tab:rq4_comparison_dimensions_overall}
\centering
\scriptsize
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{1.1}
\resizebox{\linewidth}{!}{%
\begin{tabular}{l|r|r|r|r|r|r|r|r}
\hline
\textbf{Original category} & \textbf{Posts} & \textbf{Share} & \textbf{Neg.} & \textbf{Neu.} & \textbf{Pos.} & \textbf{Mean views} & \textbf{Mean likes} & \textbf{Mean comments}\\
\hline
Usability \& Access & 233 & 56.0\% & 91 (39.1\%) & 114 (48.9\%) & 28 (12.0\%) & 1{,}524 & 2.78 & 4.15\\
Functionality \& Capabilities & 123 & 29.6\% & 55 (44.7\%) & 51 (41.5\%) & 17 (13.8\%) & 649 & 2.21 & 3.25\\
General Experience & 23 & 5.5\% & 6 (26.1\%) & 13 (56.5\%) & 4 (17.4\%) & 2{,}111 & 6.09 & 7.96\\
Pricing \& Plan & 16 & 3.8\% & 7 (43.8\%) & 8 (50.0\%) & 1 (6.3\%) & 578 & 1.19 & 3.25\\
Future Suggestions & 8 & 1.9\% & 1 (12.5\%) & 4 (50.0\%) & 3 (37.5\%) & 973 & 1.75 & 3.50\\
Performance \& Resource Usage & 5 & 1.2\% & 5 (100.0\%) & 0 (0.0\%) & 0 (0.0\%) & 879 & 2.40 & 4.00\\
Dependability \& Stability & 4 & 1.0\% & 3 (75.0\%) & 0 (0.0\%) & 1 (25.0\%) & 443 & 3.00 & 2.25\\
Privacy \& Security & 4 & 1.0\% & 0 (0.0\%) & 4 (100.0\%) & 0 (0.0\%) & 1{,}269 & 2.25 & 3.75\\
\hline
\end{tabular}%
}
\end{table}

==> tabs/neg_by_category.tex <==
\begin{table}[t]
  \caption{Sentiment by high-level category. For each category, we report the number of posts, the number of posts labeled negative, and the resulting proportion of negative posts.}  
  \label{tab:neg_sentiment_category}
  \centering
  \begin{tabular}{lrrr}
    \hline
    Category & \#~Posts & \#~Negative & \% Negative \\
    \hline
    Functionality \& Capabilities & 6{,}271 & 2{,}560 & 40.8\\
    Usability \& Access & 4{,}035 & 1922 & 47.6\\
    Pricing \& Plan & 1{,}395 & 629 & 45.1\\
    Dependability \& Stability & 800 & 547 & 68.4\\
    Performance \& Resource Usage & 446 & 396 & 88.8\\
    General Experience & 782 & 169 & 21.6\\
    Comparison & 416 & 168 & 40.4\\
    Privacy \& Security & 305 & 150 & 49.2\\
    Future Suggestions & 264 & 29 & 11.0\\
    \hline
  \end{tabular}
\end{table}

==> tabs/neg_by_forum.tex <==
\begin{table}[t]
  \caption{Negative sentiment by forum section.}  
  \label{tab:neg_sentiment_forum}
  \centering
  \begin{tabular}{lrrr}
    \hline
    Forum section & \#~Posts & \#~Negative & \% Negative \\
    \hline
    Discussions & 7{,}879 & 3947 & 50.1\\
    Bug Reports & 972 & 949 & 97.6\\
    Feature Requests & 3{,}449 & 603 & 17.5\\
    Feedback & 918 & 585 & 63.7\\
    How To & 1{,}496 & 486 & 32.5\\
    \hline
  \end{tabular}
\end{table}

==> tabs/neg_high_attention.tex <==
\begin{table}[t]
  \caption{Negative-topic hotspots by per-post attention signals}
  \label{tab:rq3_high_high}
  \centering
  \scriptsize
  \setlength{\tabcolsep}{3.5pt}
  \renewcommand{\arraystretch}{1.05}
  \begin{tabular}{>{\raggedright\arraybackslash}p{4.6cm}rrrr}
    \hline
    Subcategory & \#~Neg. & \makecell{Popularity\\(Views)} & \makecell{Agreement\\(Likes)} & \makecell{Engagement\\(Comments)} \\
    \hline
    Education, Student \& Business Packages & 8   & 1451.6 & 3.75 & 1.50 \\
    With AI coding assistants               & 23  & 1383.5 & 4.52 & 2.17 \\
    API Keys \& Connectivity                & 186 & 1216.6 & 2.17 & 2.04 \\
    Accounts, Login, Sync \& Access Control & 256 & 810.4  & 3.17 & 2.08 \\
    Plan Structure, Pricing \& Value        & 63  & 785.7  & 5.25 & 2.32 \\
    Billing, Pricing, Credits \& Payments   & 542 & 671.4  & 4.75 & 2.70 \\
    \hline
  \end{tabular}
\end{table}


==> tabs/position_cursor.tex <==
% \begin{table}[t]
%   \caption{Usage posture by stance: total posts, positive posts, and share of positive posts.}
%   \label{tab:stance_distribution}
%   \centering
%   \begin{tabular}{lrrr}
%     \hline
%     Stance & \#~Posts & \#~Positive & \% Positive \\
%     \hline
%     Primary-IDE & 2{,}417 & 797 & 33.0\\
%     Non\_primary\_tool & 1627 & 214 & 13.2\\
%     Trial-blocked & 566 & 13 & 2.3\\
%     Unclear & 10{,}104 & 1{,}591 & 15.7\\
%     \hline
%   \end{tabular}
% \end{table}

\begin{table}[t]
  \caption{Usage posture by stance: prevalence in the corpus and where positive posts originate.}
  \label{tab:stance_distribution_enriched}
  \centering
  \scriptsize
  \begin{tabular}{lrrrrr}
    \hline
    Stance & \# Posts & \% of all posts & \# Positive & \% Positive & \% of all positive \\
    \hline
    Primary-IDE       & 2{,}417  & 16.4 & 797  & 33.0 & 30.5 \\
    Non-primary tool  & 1{,}627  & 11.1 & 214  & 13.2 & 8.2 \\
    Trial-blocked     & 566      & 3.8  & 13   & 2.3  & 0.5 \\
    Unclear           & 10{,}104 & 68.7 & 1{,}591 & 15.7 & 60.8 \\
    \hline
    Total             & 14{,}714 & 100.0 & 2{,}615 & 17.8 & 100.0 \\
    \hline
  \end{tabular}
\end{table}


==> tabs/problem_type.tex <==
\begin{table}[t]
  \centering
  \caption{Problem Types of posts by forum category}
  \label{tab:problem_type}
  \scriptsize
  \setlength{\tabcolsep}{4.5pt}
  \renewcommand{\arraystretch}{1.2}
  \begin{tabular}{lrrrrrr}
    \toprule
    Category & Bug & Feature req. & Question & Performance & Feedback & Other \\
    \midrule
    Bug Reports      & 904  & 6    & 8   & 44  & 8   & 2  \\
    Feature Requests & 142  & 3152 & 93  & 13  & 47  & 2  \\
    Feedback         & 320  & 185  & 88  & 69  & 246 & 10 \\
    Discussions      & 2635 & 800  & 2894 & 332 & 1078 & 140 \\
    How To           & 351  & 241  & 735 & 23  & 112 & 19 \\
    \bottomrule
  \end{tabular}
\end{table}

==> tabs/sentiment_by_category.tex <==
\begin{table}[t]
  \caption{Sentiment by high-level category: counts and percentages of positive (green) and negative (orange) posts.
  % For each category, we report the number of posts, the number of posts labeled positive (green column) and negative (orange column), and the resulting proportion of positive and negative posts.
  }
  \label{tab:sentiment_category}
  \centering
  \scriptsize
  \setlength{\tabcolsep}{3.5pt}
  \renewcommand{\arraystretch}{1.08}

  \newcolumntype{Y}{>{\raggedright\arraybackslash}X}
  \newcolumntype{g}{>{\columncolor{green!15}}r}
  \newcolumntype{o}{>{\columncolor{orange!15}}r}

  \begin{tabularx}{\columnwidth}{Y r g r o r}
    \hline
    \textbf{Category} & \textbf{\#~Posts} & \textbf{\#~Positive} & \textbf{\% Positive} & \textbf{\#~Negative} & \textbf{\% Negative} \\
    \hline
    Functionality \& Capabilities & 6{,}360 & 1{,}338 & 21.0 & 2{,}576 & 40.5\\
    Usability \& Access & 4{,}035 & 566 & 14.0 & 1{,}922 & 47.6\\
    General Experience & 782 & 328 & 41.9 & 169 & 21.6\\
    Future Suggestions & 175 & 98 & 56.0 & 13 & 7.4\\
    Pricing \& Plan & 1{,}395 & 113 & 8.1 & 629 & 45.1\\
    Dependability \& Stability & 800 & 98 & 12.3 & 547 & 68.4\\
    Comparison & 416 & 54 & 12.98 & 168 & 40.4\\
    Privacy \& Security & 305 & 13 & 4.3 & 150 & 49.2\\
    Performance \& Resource Usage & 446 & 7 & 1.6 & 396 & 88.8\\
    \hline
  \end{tabularx}
\end{table}


==> tabs/severity.tex <==
\begin{table}[t]
  \centering
  \caption{Severity of posts by forum category}
  \label{tab:sentiment_by_category}
  \begin{tabular}{lrrrrr}
    \toprule
    Forum Category & Critical & High & Medium & Low \\
    \midrule
    Bug Reports      & 82 & 337 & 426  & 127 \\
    Feature Requests & 10  & 382 & 1661 & 1396 \\
    Feedback         & 25 & 221 & 339  & 333 \\
    Discussions      & 163 & 1550 & 2599 & 3567 \\
    How To           & 7 & 155 & 569  & 750 \\
    \bottomrule
  \end{tabular}
\end{table}

==> tabs/stance_over_time.tex <==
\begin{table}[t]
\caption{Usage posture over time: share of posts in each stance for each calendar quarter (\%).}
\label{tab:stance_quarter}
\centering
\scriptsize
\begin{tabular}{lrrrr}
\hline
Quarter & Primary-IDE & Non-primary tool & Trial-blocked & Unclear \\
\hline
2023Q3 & 13.0 & 7.7  & 1.0 & 78.3 \\
2023Q4 & 11.1 & 13.2 & 4.5 & 71.1 \\
2024Q1 & 11.1 & 11.6 & 3.4 & 73.8 \\
2024Q2 & 10.9 & 9.1  & 3.7 & 76.4 \\
2024Q3 & 12.8 & 11.3 & 3.9 & 72.0 \\
2024Q4 & 13.5 & 11.3 & 4.5 & 70.6 \\
2025Q1 & 15.1 & 11.6 & 4.0 & 69.3 \\
2025Q2 & 16.5 & 11.0 & 2.6 & 69.9 \\
2025Q3 & 17.6 & 11.9 & 3.1 & 67.4 \\
2025Q4 & 26.6 & 9.2  & 5.4 & 58.8 \\
\hline
\end{tabular}
\end{table}


==> tabs/stance_tenure.tex <==
\begin{table}[t] 
\caption{Usage posture by user tenure: share of posts in each stance as a function of days since first post (\%).} 
\label{tab:stance_tenure} 
\centering 
\scriptsize 
\begin{tabular}{lrrrr} 
\hline 
Tenure bucket & Primary-IDE & Non-primary tool & Trial-blocked & Unclear \\ 
\hline 
0--7 days & 15.8 & 11.1 & 4.3 & 68.7 \\
8--30 days & 15.3 & 12.1 & 3.9 & 68.7\\
31--90 days & 18.2 & 11.4 & 2.4 & 68.0\\ 
$>$90 days & 18.8 & 9.9 & 2.6 & 68.8\\
\hline 
\end{tabular}
\end{table}
